Revisiting Vision-Language Features Adaptation and Inconsistency for Social Media Popularity Prediction

Social media popularity (SMP) prediction is a complex task involving multi-modal data integration. While pre-trained vision-language models (VLMs) like CLIP have been widely adopted for this task, their effectiveness in capturing the unique characteristics of social media content remains unexplored. This paper critically examines the applicability of CLIP-based features in SMP prediction, focusing on the overlooked phenomenon of semantic inconsistency between images and text in social media posts. Through extensive analysis, we demonstrate that this inconsistency increases with post popularity, challenging the conventional use of VLM features. We provide a comprehensive investigation of semantic inconsistency across different popularity intervals and analyze the impact of VLM feature adaptation on SMP tasks. Our experiments reveal that incorporating inconsistency measures and adapted text features significantly improves model performance, achieving an SRC of 0.729 and an MAE of 1.227. These findings not only enhance SMP prediction accuracy but also provide crucial insights for developing more targeted approaches in social media analysis.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> old/smpd19-body.tex <==
% !TeX spellcheck = en_US
\section{Introduction}

With the rapid growth of social media in different social network platforms such as Facebook, Pinterest, Flickr, and Instagram, how to effectively predict the attractiveness of a post in the social networks becomes a critical issue. A post in a social media, however, consisting of various types of data such as the title, tags, category, descriptions, image, and meta-data. It is hard to directly apply an existing regression model to handle these heterogeneous data. A practical multi-modal prediction approach for social media is, therefore, highly desired.

%% Introduction to some regression tools

Social media prediction problem can be regarded as a regression problem. Rather than traditional machine learning-based regression models, recent ensemble learning-based approaches have shown superior performance in regression for various tasks. For example, the popularity prediction approach proposed in \cite{hsu2018social} and \cite{hsu2017social} used an ensemble regressor to achieve the iterative refinement for social media headline prediction. In addition, some advanced ensemble learning methods such as random forest \cite{rfr}, eXtreme Gradient Boosting (XGBoost) \cite{xgboost}, and LightGBM \cite{lightgbm} have been also widely used in various research fields and applications. To achieve better performance in regression and classification, an advanced approach based on the gradient boosted decision tree (GBDT), called XGBoost \cite{xgboost}, is proposed. However, the computational complexity of XGBoost is relatively high, compared with that of the random forest. Recently, LightGBM \cite{lightgbm} is proposed to overcome the shortcoming of XGBoost by replacing the level-growth tree with the leaf-growth tree. Both of XGBoost and LightGBM, however, still fail to predict the popularity from heterogeneous social media data. 
%% Introduction to some existing models ==> for SMP
\begin{figure*}
	\centering
	\includegraphics[width=0.9\textwidth]{flowchart.png}
	\caption{Flowchart of the proposed regression model with multi-modal feature mining}
	\label{fig:flowchart}	
\end{figure*}

As described above, the general ensemble learning methods cannot deal with multi-modal data (consisting of data types of text, scalar, and image raw data) directly. Effective regression for the heterogeneous data from social media remains a challenge. In \cite{hsu2017social}, social media data can be categorized into two types: 1) image data and 2) others, including text-based and numerical-based data. Based on \cite{hsu2017social} (with the goal for predicting the view count of a given post including photo and its social information), the text-based features can be simply extracted by calculating the length of each sentence. In addition, a random forest regressor is used to predict the initial popularity score for the transformed meta-data. To boost the performance, a CNN (convolution neural network) is used to predict the residual value to compensate the initial prediction for extreme high/low view counts. However, it was not addressed in \cite{hsu2017social} which feature is relatively important and highly relevant with the popularity score. Furthermore, a similar approach was also presented in \cite{hsu2018social}. To further improve the performance, an iterative residual compensation process was adapted to refine the initially predicted result. Moreover, in \cite{li2018effective}, an effective text-based feature engineering method was proposed for social media headline prediction. It also demonstrated that a proper feature engineering of social media can achieve a promising prediction result. However, how to process image data and how it affects the popularity prediction were not well addressed in \cite{li2018effective}. 

%% After some discussions of shortcomings of existing model...show some import issue
In summary, two primary issues obtained by exploring the existing approaches in social media prediction are described as follows.
\begin{itemize}
    \item No approach is currently available yet to adequately explore the multi-modal data and discover their benefits for popularity prediction. 
    \item No multi-modal learning approach relying on all types of social media data has been presented yet for popularity prediction. 
\end{itemize}

In this paper, we propose a multi-modal feature mining framework, including semantic image feature extraction and meta-data transformation to better capture the potential relationship between a social media post and its popularity score. Most of the data types used in the social media post will be through the preprocessing process, such as transformation or feature extraction, before being utilized, except for the numerical data which can be directly used. The categorical information will be encoded into a one-hot vector. Meanwhile, we adopt the image captioning approach presented in \cite{captioning} to learn the captioning model from MS-COCO\cite{coco} and predict the caption of the image of the social media post. Afterward, the text-based data will be used to train a word-to-vector model, and the trained model will be used to encode the text-based data, including image captions. Then, all kinds of processed data will be concatenated into a feature vector. Finally, LightGBM is used to learn the regression model, which is used to make the prediction on the test dataset provided by \cite{Wu2017DTCN}. The contribution of this paper is two-fold:
\begin{itemize}
    \item We present a multi-modal feature fusion framework to characterize multiple types of features, including image feature, text information, and meta-data, in an effective manner for the prediction of social media popularity.
    \item The proposed image semantic features would be beneficial to boost the performance of social media prediction task further.
\end{itemize}

The rest of this paper is organized as follows.
Section 2 presents the proposed multi-modal feature mining approach for social media popularity prediction. In Sec. 3, experimental results are demonstrated. Finally, conclusions are drawn in Sec. 4.

\section{Proposed Multi-Modal Feature Mining Framework}
\subsection{Overview of The Proposed Regression Method}

In this paper, we propose to apply LightGBM to learn the popularity prediction for social media based on the proposed multi-modal feature mining techniques. The flowchart of the proposed regression model is depicted in \ref{fig:flowchart}. First, social media data can be categorized into the four types: 1) image, 2) numerical, 3) text-based, and 4) categorical data. Each data type will have its own representation producer to obtain the final feature representation for the data. Afterward, the feature concatenation is used to fuse all processed features, and the LightGBM technique is used to train the regression model. Finally, the trained LightGBM model is used to predict the popularity score for each post in the testing social media data. The proposed multi-modal feature mining strategies will be elaborated in detail in the following sub-sections. 


\subsection{Data Preprocessing and Analysis}
Given a post of the social information $\mathbf{X}$ with $15$-dimensional vector including numerical and text-based data, the goal is to predict its popularity score. The data can be categorized into the three types:
\begin{itemize}
    \item 6 items of the numerical data: User-id (\textit{UID}), post-id (\textit{PID}), date of the post (Postdate), and geographic information (\textit{Latitude}, \textit{Longitude}, and \textit{Geoaccuracy})
    \item 6 items of the text-based data: Type of the post (\textit{Category}, \textit{Subcategory}, and \textit{Concept}), the title of the post (\textit{Title}), all tags of the post (\textit{Alltags}), and the user-defined aliasing (\textit{Pathalias})
    \item 3 items of the categorical data: The media type of the post (\textit{Mediatype}), whether the post is public (\textit{isPublic}), and whether the media is ready for access (\textit{Mediastatus}).
\end{itemize}
  The goal of the popularity prediction of social media is to predict the click count of a post based on all possible social media information, except \textit{UID} and \textit{PID} because they may be not available in the training set. In the following sub-sections, we will describe how to process and analyze the three types of data in detail. 
%%% Analyze features...
\subsubsection{Numerical Data Analysis}
The numerical data within a social media post can be directly transferred into the data of computable data type. However, their numerical ranges may be significantly different from each other. For example, the value of \textit{PID} will be from a thousand to hundreds of thousand while that of \textit{Geoaccuracy} will be from $16$ to $1$. Directly transferring these numerical data may lead to ineffective learning of the regression model. Therefore, it is necessary to carefully analyze and transfer these numerical data for improving the performance of the regression task. The post-identity data, \textit{UID} and \textit{PID}, are both in the integer form. The \textit{PID} is unique for indicating the identity of a post in a social media, whereas a user specified by \textit{UID} may have multiple posts on the social media. In our framework, \textit{UID} and \textit{PID} are only used in the implementation stage to link the data (of different types and distributed among different files) belonging to the same post. Both of them are not involved in the model training stage. As suggested by \cite{hsu2018social}, a unique number representation manner is efficient for representation of the \textit{UID} and \textit{PID} data.

In our method, the published date of a post, \textit{Postdate}, is encoded in a time-stamp format. We assumed that the date of the post would relate to its popularity score. For example, the number of people exploring a social media platform at night would be more than that at day. In addition, more people would prefer to join the social media platform at weekend than those at working days. To better reflect these observations from the \textit{Postdate}, we transfer the Postdate item into the five sub-items, i.e., hour, week, day, month, and year, denoted as 
\begin{equation}
    \mathbf{f}_{time}=[f_{hour},f_{week},f_{day},f_{month},f_{year}].
\end{equation}

Moreover, the geographic information - \textit{Latitude} and \textit{Longitude} - are ranged from -90 to 90 degrees and from -180 to 180 degrees, respectively. A common example for the usage of geographic information is that a post of specified famous tourist attraction may have higher click count, which can be characterized by {Latitude} and {Longitude} directly. In our method, both of them are transformed into the data of floating point type without preprocessing. In addition, the \textit{Geoaccuracy} indicates the trust degree of \textit{Latitude} and \textit{Longitude} information. Here, we transfer it into the data of integer type directly. Therefore, the final geographic information can be denoted as 
\begin{equation}
    \mathbf{f}_{Geo} = [f_{Latitude}, f_{Longitude}, f_{Geoaccuracy}].
\end{equation}
\subsubsection{Text-based Data Analysis}
Since the count of the characters significantly varies with different text-based information, it is hard to transfer it into fixed-length data. As described in \cite{hsu2018social}, the most straightforward way to deal with the text-based data transformation is to calculate the number of words. Inspired by \cite{li2018effective}, the text-based information can be effectively represented by word-to-vector model \cite{word2vec}.  

Different from \cite{li2018effective}, we, respectively, create word-to-vector models for \textit{Alltags} $\mathbf{f}_{Alltags}$ and the other text-based data (including \textit{Category}, \textit{Subcategory}, \textit{Concept}, and \textit{Pathalias}) in order to better characterize text-based information. For the sake of convenience, the other text-based data can be denoted as
\begin{equation}
\mathbf{f}_{text} = [f_{Cat}, f_{Subcat}, f_{Concept}, f_{Pathalias}].
\end{equation}
 
On the other hand, since $f_{Alltags}$ is more complicated than the other text-based information, it would be better to learn its word-to-vector model with larger vector size, compared to $\mathbf{f}_{text}$. Finally, the trained models $Wb_{Alltags}$ and $Wb_{text}$ can be used to encode the text-based information as follows:
\begin{equation}
\begin{split}
    \textbf{f}_{w2v}^1 = Wb_{Alltags}(\mathbf{f}_{Alltags}), and\\
    \textbf{f}_{w2v}^2 = Wb_{text}(\mathbf{f}_{text}).
\end{split}
\end{equation}
\begin{figure*}
	\centering
	\includegraphics[width=0.85\textwidth]{image_vs_count.png}
	\caption{The image information of two posts in the social media with (a) high popularity score (13.3) and (b) low popularity score (3.5)}
	\label{fig:ex1}	
\end{figure*}

\subsection{Categorical Data Analysis}
In the categorical data including \textit{Mediatype}, \textit{Mediastatus}, and \textit{isPublic}, they need to be represented in different forms from each other. For instance, the feature \textit{Mediastatus} is encoded by text where the "ready" indicates that the attached media of the post is ready for access, while the feature \textit{isPublic} uses 0 or 1 to denote whether the post is publicly accessible or not. To well represent the categorical data, the data will be encoded as a one-hot vector representation, as follows:
\begin{eqnarray}
    \textbf{f}_{OH}^{type} = One_Hot_Encoding(f_{type}),
\end{eqnarray}
where $type$ is one of \textit{Mediatype}, \textit{Mediastatus}, and \textit{isPublic}.

In addition to the social media information provided by \cite{Wu2017DTCN}, most of the posts also contain pictures. However, the image data type is quite different from those of the other social media data. It is hard to feed image data to any existing regression models directly. To tackle this problem, we propose an image semantic feature extraction method to effectively explore the potential relationship between the image and the popularity score of the corresponding post, as described in the following sub-section.

\subsection{Image Semantic Feature Extraction}

As presented in \cite{hsu2017social}, image data of a post can be used to predict the residual between the initially predicted popularity obtained by the random forest technique and that of the ground truth. However, it was not well analyzed how the photo-style affects the popularity of a post so that the impact of image data for popularity remains an open problem. As shown in Fig. \ref{fig:ex1}, some minor cues may be found for image information to recognize what type of image content would have a high popularity and vice versa. Based on our extensive observations on the images of social media posts, we have found that life photo-like images would usually lead to lower popularity score. However, there is no image-style label available in the images on social media so that it is hard to adopt the image-style as a feature for popularity prediction. 

Fortunately, the image-style information may be captured by some semantic feature. For example, different image styles can be regarded as different combinations of the objects in the images. To capture such kind of feature, in this study, we introduce the image captioning model SAT (Show, Attention, and Tell) in \cite{captioning} to extract the semantic feature. To achieve better performance of SAT model, the backbone network in SAT is replaced with the Neural Architecture Search (NAS) \cite{nas}, as well as the size of the input image to SAT, is enlarged to $331\times331$. We train the SAT on MS-COCO with Adam optimizer. Afterward, the learned SAT is used to predict the captioning of the image within a social media post. Similarly, the caption of an image can be encoded by the word-to-vector model $ Wb_{Caption}$, as follows:
\begin{eqnarray}
    \textbf{f}_{w2v}^3 = Wb_{Caption}(\mathbf{f}_{Caption}).
\end{eqnarray}

The image captioning feature can be regarded as a high-level feature. However, there may exist some objects in MS-COCO that cannot be found in SMD. Therefore, only image captioning-based feature for popularity prediction may be ineffective for some cases. To solve this, we also propose to retrieve the middle-level feature $\textbf{f}_{imfeat}$ from the last layers in the CNN-encoder adopted in SAT. However, the feature dimension is somewhat relatively high (say, 2048 dimensions), compared to the other features in SMD. To solve this problem, the Principal Component Analysis (PCA) \cite{pca} technique is used to reduce the feature dimension. Assumed that $\textbf{C}$ is the covariance matrix of the image feature matrix $\textbf{F}_{imfeat}=[\textbf{f}_{imfeat}^1,...,\textbf{f}_{imfeat}^N]$, where $N$ is the number of posts in SMD. The projection matrix $\textbf{v}$ can be obtained by solving
\begin{eqnarray}
    \textbf{v}=\arg\max_{||\textbf{v}||=1} \textbf{v}^{T}\textbf{Cv}.
\end{eqnarray}
The encoded middle-level feature can be obtained by
\begin{eqnarray}
    \textbf{f}_{im_PCA} = {F}_{imfeat}\times v.
\end{eqnarray}

Afterward, the multi-modal feature is defined as follows:

\begin{equation}
\begin{split}
    &\mathbf{F}_{merged} = \\
    &[\mathbf{f}_{time}, \mathbf{f}_{Geo}, \mathbf{f}_{text}, \mathbf{f}_{OH}^{type}, \mathbf{f}_{w2v}^1, \mathbf{f}_{w2v}^2, \mathbf{f}_{w2v}^3, \mathbf{f}_{im_PCA}],\\
    &type\in\{\textit{Mediatype}, \textit{Mediastatus}, \textit{isPublic}\}.
\end{split}
\end{equation}
Finally, the popularity score of SMD can be successfully predicted based on the proposed multi-modal feature $\mathbf{F}_{merged}$ by LightGBM \cite{lightgbm}.

\section{Experimental Results}
\subsection{Experimental Settings}
In our experiments, SMD consisting of $305,614$ posts \cite{Wu2017DTCN}\cite{Wu2016TemporalPrediction}\cite{Wu2016TimeMatters} is used to evaluate the performance of the proposed popularity prediction framework, compared with the other state-of-the-art methods. In the used SMD (the data from Flickr), some images are set to be inaccessible, and only $275,066$ images in total are available. By observing the released testing set, there are $1/3$ posts' \textit{UID} that did not exist in SMD. To effectively verify the performances of the evaluated methods, the dataset in SMD is further partitioned into a training set and a testing set, including $300,000$ and $5,614$ posts, respectively, where the \textit{UIDs} in the training set and the testing set are isolated. The employed metrics for performance evaluation include Spearman's Rho rank correlation (SRC)\cite{rc}, Mean Absolute Error (MAE), and Mean Squared Error (MSE), where the rank correlation is a non-parametric measurement of statistical dependence between the rankings of two variables.

The batch size used in the image captioning SAT model is 24, and the middle-level feature size in CNN-encoder is $2,048$. The trained PCA is used to project the middle-level feature into the $50$-dimension data vector. There are three word-to-vector models for encoding \textit{Alltages}, the other text-based data, and the caption data. The lengths of the encoded vectors of these three word-to-vector models are $50$, $20$, and $20$, respectively. 

To evaluate the performance of the proposed popularity prediction method, we collected the seven state-of-the-art regression methods for comparisons, described as follows:
\begin{itemize}
	\item Multi-Model (MM) method proposed in \cite{hsu2017social}.
	\item Iterative Refinement (IR) method proposed in \cite{hsu2018social}.
	\item Effective Word Encoding (EWE) method proposed in \cite{li2018effective}.
	\item Feature preprocessing (Baseline-I) method presented in \cite{hsu2017social} + XGBoost.
	\item Feature preprocessing (Baseline-II) method presented in \cite{hsu2018social} + XGBoost.
	\item Feature preprocessing (Baseline-III) method presented in \cite{hsu2017social} + LightGBM.
	\item Feature preprocessing (Baseline-IV) method presented in \cite{hsu2018social} + LightGBM.
\end{itemize}
Note, all of the parameters used in these compared methods were set to the corresponding values suggested by the respective papers accordingly.

\subsection{Performance Comparison}
\begin{table}
  \caption{Performance comparison among the different regression methods evaluated on the testing set}
  \label{tab:exp1}
  \begin{tabular}{cccc}
    \toprule
    Methods &  SRC & MSE & MAE \\
    \midrule
    Baseline-I 	                & 0.448 & 7.595 & 2.107\\
    Baseline-II         	    & 0.450 & 5.411 & 1.846 \\
    Baseline-III        	    & 0.461 & 5.068 & 1.785 \\
    Baseline-IV                 & 0.470 & 5.442 & 1.871 \\
    MM \cite{hsu2017social}     & 0.528 & 5.891 & 1.942 \\
    IR \cite{hsu2018social}     & 0.537 & 5.872 & 1.939 \\
    EW \cite{li2018effective}	& 0.548 & 5.856 & 1.938 \\
    Proposed                    &$\mathbf{ 0.656}$ & $\mathbf{3.561}$ & $\mathbf{1.497}$ \\
  \bottomrule
\end{tabular}
\end{table}
As shown in Table \ref{tab:exp1}, the proposed method significantly outperforms the other state-of-the-art methods used for comparisons in terms of SRC, MSE, and MAE. Compared to the previous prediction models proposed in \cite{hsu2017social}\cite{hsu2018social}, it has been demonstrated that proper data preprocessing would be effective for boosting the prediction performance. In \cite{li2018effective}, the text-based features were also encoded by the word-to-vector models. However, the other data types (say, image, numerical, and categorical features) in the social media were not well addressed in \cite{li2018effective}, leading to suppressed results. We also replaced the data processing strategies of the proposed method with the strategies presented in \cite{hsu2017social}\cite{hsu2018social} to form the four baseline models used for comparisons. The proposed method has shown the superior performance to verify the effectiveness of the proposed multi-modal feature mining approach.

\subsection{Ablation Study}
To perform ablation study, we removed different terms from the proposed framework to verify the importance and contribution of each component in the proposed multi-modal feature mining method. The components of the numerical data processing, the text-based data processing, the high-level image feature extraction, and the middle-level image feature extraction are, respectively, denoted by $N$, $T$, $C$, and $I$. The different combinations among them were performed for the performance comparisons in the ablation study, as shown in Table \ref{tab:exp2}. It should be noted that the most important feature is still the meta-data. However, it has been shown that the combination of text-based feature and numerical data can effectively boost the performance, as also proved by \cite{li2018effective}. By mining more critical features from the image of a post, the fused feature can further improve the performance of the prediction for popularity score. In conclusion, the proposed multi-modal data mining approach has been shown to be effective in fusion of multiple types of social media data, which is beneficial for accurate prediction of popularity for the social media posts. 
\begin{table}
  \caption{Performance evaluation for the ablation study of the proposed method}
  \label{tab:exp2}
  \begin{tabular}{cccc}
    \toprule
    Methods &  SRC & MSE & MAE \\
    \midrule
    Baseline-III        	    & 0.461 & 5.068 & 1.785 \\
    Baseline-IV                 & 0.470 & 5.442 & 1.871 \\
    $N$ only  	                & 0.310 & 5.391 & 1.872\\
    $T$ only  	                & 0.605 & 4.002 & 1.572\\
    $C$ only  	                & 0.114 & 5.969 & 1.954\\
    $I$ only  	                & 0.185 & 5.803 & 1.930\\
    $N+T$         	            & 0.622 & 3.993 & 1.588 \\
    $N+C$         	            & 0.331 & 5.268 & 1.849 \\
    $N+I$         	            & 0.372 & 5.081 & 1.815 \\
    $N+T+C$     	            & 0.646 & 3.653 & 1.514 \\
    $N+T+I$     	            & 0.652 & 3.601 & 1.503\\
    $N+C+I$         	        & 0.376 & 5.049 & 1.810 \\
    $T+C$         	            & 0.600 & 4.026 & 1.577 \\
    $T+C+I$         	        & 0.611 & 3.940 & 1.552 \\
    $T+I$         	            & 0.608 & 3.976 & 1.561\\
    $C+I$         	            & 0.195 & 5.768 & 1.923 \\
    Proposed $N+T+C+I$          &$\mathbf{ 0.656}$ & $\mathbf{3.561}$ & $\mathbf{1.497}$ \\
  \bottomrule
\end{tabular}
\end{table}

\section{Conclusions}
In this paper, we have proposed a multi-modal feature mining framework that can effectively discover the useful features from social media. We also showed that well-processed text-based mining would be beneficial to popularity prediction. Furthermore, we have proposed an image semantic feature extraction approach to extract both of the high-level and middle-level features from the attached image of the post, which significantly enhances the popularity prediction performance further. Extensive experiments have demonstrated that the proposed multi-modal feature mining model can achieve state-of-the-art performance in terms of various metrics.
\begin{acks}
This study was supported in part by the Ministry of Science and Technology, Taiwan, under Grants MOST 108-2634-F-007-009, 107-2218-E-020-002-MY3, 107-2218-E-006-059, 108-2221-E-224-024-MY3, and 105-2628-E-224-001-MY3.
We thank SMP Challenge organizers for providing the large-scale social media dataset.
\end{acks}

==> smpd23-acmmm.tex <==
% !TeX spellcheck = en_US

\section{Introduction}

In recent years, people have preferred using social media to share their daily lives and engage in marketing activities, thereby leveraging their personal or brand influence. In other words, social media platforms hold immense value. Consequently, the accurate analysis of social media and user behavior has emerged as a burgeoning research topic. 

Social media platforms encompass various types of data, posing challenges in accurately predicting SMP tasks due to the complexity of feature combinations. Appropriate feature transformations are critical for handling different feature types. Previous studies have been limited by weak feature extractors, hindering the improvement of task baselines. 

In methodologies development, several prior arts have been proposed in recent years for SMP tasks. The peer methods in \cite{hsu2018social, hsu2019social, hsu2020social} models treat the prediction task in SMP as a multi-modal regression task. For feature extraction, conventional natural language processing (NLP) models are typically employed to obtain semantic features from text information, such as RoBERTa \cite{liu2019roberta} and Sentence-Transformer \cite{reimers-2019-sentence-bert}. In \cite{hsu2019social}, it is claimed that incorporating image features and generative captions can further improve the performance of the SMP task. Some recent state-of-the-art, such as \cite{lastyear1}\cite{lastyear2}\cite{lastyear3}, have integrated multi-modal features and external user information, reaching outstanding performance in SMP tasks. However, lacking comprehensive study on the impact of external identity-related features results in difficulty in further improving performance. We, therefore, provide a complete discussion and experiments on discovering how the identity-related features important is.

Specifically, HyFea\cite{10.1145/3394171.3416273}, proposed by Lai et al., highlights that we can obtain additional user profile data, such as totalViews (#counts of viewers) and totalFollowing (How many users follow the targeted user). Mining additional features correlated with the user (identity) can enrich user information, thereby improving the performance of SMP tasks. We conduct a series of experiments to investigate its correlation. Specifically, the external identity-related feature reflects the characteristics of an "internet celebrity." Posts from internet celebrities are often more likely to attract attention, thereby affecting the popularity of their posts.

However, in traditional SMP tasks \cite{smp1, smp2, smp3}, data was typically split into training and testing sets based solely on the timestamp. This approach needed to account for potential user differences between the sets. As user identity plays a crucial role in SMP tasks \cite{hsu2018social, hsu2019social, hsu2020social,10.1145/3503161.3551593}, improper data splitting methods could result in missing UIDs and consequently limit the performance of the SMP task. On the one hand, the profile-related features significantly contribute to the performance of SMP tasks. On the other hand, overly relying on such identity-related features could result in bad prediction results when its identity is new. Therefore, to avoid overly focusing on user-specific details and promote a more generalized approach in SMP tasks, we utilize group k-fold validation based on the number of unique UIDs, ensuring non-overlapping users in each fold. This allows us to retain crucial user information while preventing the model from over-relying on user-specific details, striking a balance between capturing semantic information and maintaining generalizability.

To handle popularity prediction using features extracted from social media, traditional discrete regression schemes have been employed, including XGBoost (XGB) \cite{xgboost}, Random Forest (RF) \cite{rfr}, LightGBM (LGBM) \cite{lightgbm}, CatBoost (CATB) \cite{prokhorenkova2018catboost}, and even model stacking \cite{matlock2018investigation}. These supervised learning and ensemble-based strategies have demonstrated their effectiveness across various tasks, particularly in tabular data. 

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{2.featuretransform.png}
    \caption{The illustrations for the multi-modal feature transformation module(MFTM). Features are processed by specific transformation, followed by dimension reduction(PCA), and are then concatenated together.}
    \label{fig:featuretransform.png}	
\end{figure}

To earn better performance of SMP tasks, as well as fully discover the identity-related, this paper proposes a robust and reliable time-series regression framework based on multi-modal feature aggregation and external profile features mining based on extensive feature analysis. 

Firstly, we improve the previously proposed multi-modal feature aggregation module proposed in \cite{10.1145/3503161.3551593} last year by replacing it with more advantageous feature extractors. Additionally, we apply a group k-fold validation that preserves user information for prediction tasks. This setting is essential to truly and fairly evaluate the performance during the training phase. Secondly, we compare the impact of different identity-related features and other features from meta-data on popularity prediction. We analyze whether the semantic meaning of external features aligns with the semantic meaning of popularity. The contribution of this paper is threefold:
\begin{itemize}
    \item We adjust the feature transformation process and compare it with the existing module to investigate the impact of different feature combinations on the model's performance.
    \item To better observe the effect of stacking multi-modality feature, We conduct some experiments to make the ablation study to examine the influence of the different semantic representations.
    \item We discover that external identity-related features have a significant impact on the SMP task. Therefore, we conduct comprehensive experiments to observe the relationship between different identity-related features and the popularity score.
\end{itemize}
The rest of this paper is organized as follows. Section 2 presents the proposed multi-modal feature transformation and the robust prediction framework for the SMP task. Section 3 shows our experimental results. Finally, conclusions are drawn in Section 4.




\begin{figure*}
 	\centering
	\includegraphics[width=0.9\textwidth]{1.flowchart.png}
	\caption{Flowchart of the proposed regression model with multi-modal feature mining.}
	\label{fig:flowchart.png}	
\end{figure*}

\section{Advanced Analysis of Multi-modal Feature Transformation}
\subsection{Overview}
Building upon prior research, the SMP dataset houses numerous distinctive features categorized into six domains: numerical, categorical, temporal, spatial, text, and image. A key step after data extraction involves an elaborate feature transformation module to convert each feature into different-dimension embedding vectors or variable forms for a comprehensive analysis. This is visually represented in Fig. \ref{fig:featuretransform.png}. Our comprehensive analysis demonstrates that, contrary to prior assumptions, the most critical feature is profile-based, thus warranting external feature crawling.

\subsection{Detailed Feature Transform Block}
The SMP dataset exhibits considerable complexity and variability across different feature types. To navigate this complexity, we carry out targeted feature transformations, deriving diverse embedding vectors or alternative features. These transformations culminate in a comprehensive representation of a social media post.

\noindent\textbf{Image Data Analysis.}
Previous work \cite{hsu2019social} has shown that image captioning offers significant benefits for SMP tasks. Using this insight, our study leverages the instructBLIP \cite{instructblip} model in tandem with prompt engineering ("Write a detailed description") to generate descriptive image captions averaging 400 words. A pre-trained Sentence Transformer \cite{reimers-2019-sentence-bert} extracts semantic features from these captions ($f_{cap}$). Simultaneously, a pre-trained EVA02-large \cite{EVA02,rw2019timm} model coupled with PCA \cite{doi:10.1080/14786440109462720} is used for image feature extraction and dimensionality reduction ($f_{image}$).

\noindent\textbf{Numerical Data Analysis.}
The UID and post-ID (PID) are converted into unique integers, while the post publish timestamp is transformed into a DateTime variable ($f_{time}$). Spatial data such as latitude and longitude are encoded via Geocoder, transforming them into categorical variables (city, state, country) represented as $f_{geo}$.  We utilize HyFea\cite{10.1145/3394171.3416273} to get external user information data, denoted as $f_{eu}$. All external user information data is connected to UID. In other words, these features are identity-related. The remainder of the numerical data is denoted as $f_{n}$.

\noindent\textbf{Text-based Data Analysis.}
Our analysis uncovers that textual features possess multilingual attributes. To prevent performance degradation caused by single language-trained feature extractors, we use Sentence Transformers \cite{reimers-2019-sentence-bert, reimers-2020-multilingual-sentence-bert} and PCA to derive $f_{multi-lang}$ and $f_{single-lang}$ representations.

\noindent\textbf{Categorical Data Analysis.}
Categorical data are represented as one-hot vector representations, denoted as $f_{cat}$.

\noindent\textbf{Multi-Modality Data Analysis.}
Since SMP dataset does not allow direct access to multi-modal features, we combine features across different modalities for extraction. Observations reveal non-overlapping semantic information between various text features. This realization leads us to pair different text types with images, generating distinct output vectors that are subsequently dimensionally reduced using PCA, resulting in the final feature representation ($f_{m}$).

\noindent\textbf{Feature Aggregation.}
Once all pertinent information is processed, we aggregate all features as $f_{all}$ = [$f_{cap}$, $f_{image}$, $f_{time}$, $f_{geo}$, $f_{n}$, $f_{eu}$, $f_{single_lang}$, $f_{multi_lang}$, $f_{cat}$, $f_{m}$] serving as the basis for social media popularity prediction.

\subsection{Group {k}-fold Validation and Prediction for Greater Robustness}
In the context of social media prediction, user-specific information significantly impacts the results. However, considering the possible lack of continuity in user presence across training and testing sets, our objective is to develop a model that can still capture the dataset's essence. Our chosen approach involves a unique group {k}-fold cross-validation where UIDs are divided into $k$ groups. This strategy increases model stability and curtails overfitting. In each fold, the model predicts the testing set's popularity. The median value of the predicted popularity scores from all folds is used for the final prediction, enhancing prediction reliability and model robustness.

\subsection{Model Ensemble Strategy for Enhanced Predictive Power}
A model ensemble leverages the predictions of multiple independent models to augment overall predictive performance and stability. This study benefits from the synergy of LightGBM \cite{lightgbm} - known for its proficiency in managing tabular data, and TabNet \cite{tabnet} - known for handling high-dimensional complex tabular data. The final prediction of social media popularity is obtained by computing a weighted average of the predictions from these two models. This ensemble strategy enhances the robustness of our model, reinforcing the importance of our findings on the critical role of profile-based features in social media popularity prediction.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experimental Results}
The SMP Dataset (SMPD), derived from \cite{smp1,smp2,smp3}, contains 305,614 posts with an array of diverse data types. As per \cite{hsu2020social}, the treatment of missing data is specific. For performance evaluation, the study utilizes Spearman's Rho rank correlation (SRC)\cite{rc} and Mean Absolute Error (MAE) as evaluation metrics.

\subsection{Performance Evaluation of the Proposed Method}
This section details the performance assessment of the traditional SMP task executed via the proposed multi-modal feature mining framework.

As delineated in Table \ref{tab:proposed method}, our strategy optimizes the prior model using findings from the 2022 SMP competition. We enrich the model by stacking external identity-related features and employing advanced feature extractors, thereby significantly outperforming the preceding model\cite{10.1145/3503161.3551593}.

Our experimental findings accentuate that supplementary identity-related features such as totalFaves, followers, and totalInGroup, exert the most substantial impact on model performance. Contrarily, other features present a comparatively restrained effect on performance, although contributing incrementally to the final result. Besides LightGBM, suitable for tabular data analysis, we integrate TabNet due to its prowess in analyzing complex semantic representations within embedding vectors. The culmination of these strategies in our model ensemble yields an SRC of \textbf{0.718} and an MAE of \textbf{1.241} for our final submission in the 2023 ACM Multimedia Social Media Prediction Challenge.


\begin{table}[htbp]
\centering
\caption{Performance comparison of proposed method based on stacking different features.}
\label{tab:proposed method}
\scalebox{0.9}{
\begin{tabular}{ccc|c|c|ccc}
\hline
& & \multicolumn{2}{c}{LGBM} & \multicolumn{2}{c}{TabNet} \\
& & SRC \uparrow & MAE  \downarrow& SRC \uparrow & MAE\downarrow \\
\hline
\multicolumn{1}{l}{The result of the SMP in 2022} & & 0.636 & 1.436 & 0.625 & 1.502 \\
\multicolumn{1}{l}{+ External Identity-related Feature} & & 0.707 & 1.261 & 0.66 & 1.362 \\
\multicolumn{1}{l}{+ Image and Text Feature} & & 0.708 & 1.26 & 0.668 & 1.366 \\
\multicolumn{1}{l}{+ Multi-modality Feature} & & 0.711 & 1.252 & 0.671 & 1.354 \\
\multicolumn{1}{l}{+ Image Captioning Feature} & & 0.713 & 1.249 & 0.682 & 1.345 \\
\hline
\end{tabular}
}
\end{table}

\subsection{Ablation Study of MFTM for SMP Task}
We acknowledge the potential for different features to variably influence model performance. In an effort to comprehend this, we orchestrate ablation experiments to explore the effects of distinct features, as tabulated in Table \ref{tab:exp3}. When utilizing image, text, and multi-modality features separately, performance is roughly equivalent. If a singular feature extractor is sufficiently potent and not fine-tuned, it is feasible to train the model solely on a single modality feature. This approach mitigates computational complexity and memory usage. However, when computational resources are copious, stacking all features potentially augments performance.

\begin{table} %%% Add 3 experiments for light-ablation study
  \caption{Ablation study about multi-modality feature transformation module for the social media prediction task.}
  \label{tab:exp3}
  \scalebox{0.85}{
  \begin{tabular}{ccccccc}
    \toprule\small
    Userprofile&Image &Text &Multimodal&Captioning  & SRC \uparrow & MAE \downarrow\\
    \midrule
    &$\surd$&  $\surd$&   $\surd$ &$\surd$	&0.65	&1.41\\
    $\surd$ &$\surd$	& & & &0.708	&1.258	\\
    $\surd$ &	& $\surd$&  & &0.708 &1.26\\
    $\surd$ &$\surd$	& $\surd$&  & &0.712 &1.251\\
    
    $\surd$ & & & $\surd$ &    $\surd$&0.709	&1.257\\
    
    $\surd$ &$\surd$ & $\surd$& $\surd$ &    &0.711	&1.252\\
    $\surd$ &$\surd$	& $\surd$&  & $\surd$ &0.711		&1.25\\
    $\surd$ &$\surd$&  $\surd$&   $\surd$ &$\surd$	&0.713	&1.249\\ 
    \bottomrule
\end{tabular}
}
\end{table}

%%%Add the latest sentence
%\begin{table} %%% Add 3 experiments for light-ablation study
%  \caption{Feature importance versus feature correlation.}
%  \label{tab:exp2}
%  \begin{tabular}{ccc}
%    \toprule\small
%    &  Importance & UID-Correlation  \\
%    \midrule
%    top1	& UID		& 1\\
%    top2	& PID		& 0.652 \\
%    top3   	& Latitude	& 0.652 \\
%    top4    & Longitude    & 0.652 \\  
%    top5	& Path-Alias    & n/a \\
%    top6    & Post Date     & 0.210 \\
%
%  \bottomrule
%\end{tabular}
%\end{table}

\begin{table}[h]
\centering
\begin{tabular}{c|c|c}
\hline\small
\textbf{Ranking}&\textbf{Variable} & \textbf{SRC(abs)} \uparrow \\
\hline
\hline
top1&Popularity score & 1 \\
\hline
top2&follower & \textbf{0.376} \\
\hline
top3&totalInGroup  & 0.31 \\
\hline
top4&totalViews & 0.30 \\
\hline
top5&following & 0.29 \\
\hline
top6&totalFaves & 0.28 \\
\hline
top7&totalTags & 0.21 \\
\hline
top8&totalGeotagged & 0.16 \\
\hline
top9&totalImages & 0.03 \\
\hline
\hline

 &Average of external features & \textbf{0.257} \\
 &Average of original features & 0.012 \\
\hline
\end{tabular}
\caption{Spearman's Rho rank Correlation Coefficient with Popularity score between external identity-related features and original numeric features.}
\label{tab:correlation}
\end{table}


%\begin{table} %%% Add 3 experiments for light-ablation study
%  \caption{Performance of the proposed model based on random split and the identity-isolated split.}
%  \label{tab:exp3}
%  \begin{tabular}{cccccc}
%    \toprule\small
%    Methods  &Uid &Pid  & SRC & MSE & MAE \\
%    \midrule
%    random split	&$\surd$ &$\surd$   &0.891	&1.320	&0.738\\
%    random split	& &$\surd$   &0.888	&1.356	&0.748\\
%    random split	& &   &0.888	&1.352	&0.748\\
%    identity-isolated split 		&$\surd$  &$\surd$    &0.680	&3.329	&1.439\\
%   identity-isolated split 		&  &$\surd$    &0.666	&3.469	&1.472\\
%   identity-isolated split 		&  &    &0.662	&3.467	&1.473\\
%  \bottomrule
%\end{tabular}
%\end{table}

\subsection{Comparison of the Influence of External Features}
Upon contrasting the correlation coefficients of these external features with the popularity score against those of the original features, we discern a more robust correlation in the former, as shown in Table \ref{tab:correlation}. This evidence suggests the identity-related features' pivotal role in predicting a post's popularity score. Further, we generate visualizations in Figure \ref{fig:corr.jpg}, projecting user profile features strongly correlating with popularity score alongside arbitrarily selected non-user profile features onto a two-dimensional plane. These visualizations depict a semantic association between user-profile features and the popularity score. In our experimental parameters, a "strong" user profile denotes a more extensive and detailed profile, while a "weak" profile suggests a less comprehensive user profile.

We observe that specific external identity-related features, indicative of user popularity and social connections within the community, wield a particularly high influence. These findings underscore the paramount importance of these external features in the determination of a post's popularity score.
 
 
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{pictures_legend_.jpeg}
    \caption{
The t-SNE visualization. The left figure shows a link between strong user profile features and popularity. The right figure shows that non-user profile features don't noticeably affect popularity}
    \label{fig:corr.jpg}	
\end{figure}

\section{Conclusions}
This paper introduces a robust multi-modality feature mining framework that amalgamates different features to capture a comprehensive range of semantic information. This comprehensive approach yields more stable predictions for social media popularity scores. The experiment substantiates the premise that \textbf{"the stronger the user profile, the more popular the posts tend to be."} We postulate that the degree of user interconnection, indicative of "Internet celebrity" behaviors, bears more influence than other features. Moreover, when contrasting different features, we ascertain that integrating more multi-modal features also provides a tangible benefit for the SMP task.
% \begin{acks}
% This study was supported in part by the Ministry of Science and Technology, Taiwan, under Grants MOST 108-2634-F-007-009, 107-2218-E-020-002-MY3, 107-2218-E-006-059, 108-2221-E-224-024-MY3, 105-2628-E-224-001-MY3, and 108-2221-E-003-027-MY3.
% We thank SMP Challenge organizers for providing the large-scale social media dataset.
% \end{acks}
